The generalized weighted probability measure on the symmetric group and the asymptotic behavior of the cycles

The goal of this paper is to analyse the asymptotic behavior of the cycle process and the total number of cycles of weighted and generalized weighted random permutations which are relevant models in physics and which extend the Ewens measure. We combine tools from combinatorics and complex analysis (e.g. singularity analysis of generating functions) to prove that under some analytic conditions (on relevant generating functions) the cycle process converges to a vector of independent Poisson variables and to establish a central limit theorem for the total number of cycles. Our methods allow us to obtain an asymptotic estimate of the characteristic functions of the different random vectors of interest together with an error estimate, thus having a control on the speed of convergence. In fact we are able to prove a finer convergence for the total number of cycles, namely \textit{mod-Poisson convergence}. From there we apply previous results on mod-Poisson convergence to obtain Poisson approximation for the total number of cycles as well as large deviations estimates.

==> section_gen_fkt.tex <==
\section{Generating functions}
\label{sec_gen_fkt}

The idea of generating functions is to encode information of a sequence into a formal power series.
We define
%
\begin{definition}
\label{def_gneranting_function}
Let $\bigl(g_n \bigr)_{n\in\N}$ be a sequence of complex numbers. We then define
%[Ordinary generating function]
%\begin{itemize}
 \item 
the (ordinary) generating function of $\bigl(g_n \bigr)_{n\in\N}$ as the formal power series
    \begin{align}
      OG(t) = OG(g_n,t) = \sum_{n=0}^\infty g_n t^n.
    \end{align}
% \item The exponential generating function of $\bigl(g_n \bigr)_{n\in\N}$ is the formal power series
%     \begin{align}
%       EG(t) = EG(g_n,t) = \sum_{n=0}^\infty \frac{g_n}{n!} t^n.
%     \end{align}
%\end{itemize}
%
\end{definition}
%
%
The exists several versions of generating functions. We use here most time only ordinary generating functions and thus call them just generating functions.
We will replace later (see Section~\ref{sec_central_limit_tot_number_cycles}) $g_n$ by holomorphic functions $g_n(w)$.
Such generating functions are then called bivariate generating functions.
We call them for simplicity also generating functions.
We need also
%
\begin{definition}
Let $OG(t) = \sum_{n=0}^\infty g_n t^n$ be a formal power series.  We then define $\nth{OG} := g_n$. \\
%We use $\nth{\cdot}$ only with respect to $t$, also when $g_n$ depends on other variables.
\end{definition}
%
%
%
%
%
%
%
%
%
The reason why generating functions are useful is that it is often possible to write down a generating function
without knowing $g_n$ explicitly. 
%
%
%
%
%
One of the main tools in this paper to write down generating functions  is
%
\begin{lemma}
\label{lem_cycle_index_theorem}
%
Let $(a_m)_{m\in\N}$ be a sequence of complex numbers. Then
%
\begin{align}
\label{eq_symm fkt}
\sla \left(\prod_{m=1}^{l(\la)} a_m\right) t^{|\la|}
=
\sla \left(\prod_{m=1}^{\infty} (a_m t^m)^{C_m} \right)
=
\exp\left(\sum_{m=1}\frac{1}{m} a_m t^m\right)
\end{align}
%
with the same $z_\la$ as in Lemma~\ref{lem_size_of_conj_classes}.\\
%
If one of the sums in \eqref{eq_symm fkt} is absolutely convergent then so are the other.
\end{lemma}
%
\begin{proof}
The first equality follows immediately from the definition of $C_m$.
The proof of the second equality in \eqref{eq_symm fkt} can be found in \cite{macdonald} or can be directly verified using the definitions of $z_\la$ and the exponential function.
The last statement follows with dominated convergence.
\end{proof}
%
We now use this lemma to show \eqref{eq_def_gen_Gt_with_hn}, i.e. $G_\Theta(t) = \sum_{n=0}^\infty h_n t^n$.
We know from \eqref{eq_PTheta_with_partition} that
%
\begin{align}
h_n
=
\frac{1}{n!} \sum_{\sigma\in S_n} \prod_{m=1}^{n} \theta_{m}^{C_m}
=
\frac{1}{n!} \sum_{\la \vdash n} \frac{n!}{z_\la} \prod_{m=1}^{l(\la)} \theta_{\la_m}
=
\sum_{\la \vdash n} \frac{1}{z_\la} \prod_{m=1}^{l(\la)} \theta_{\la_m}.
\end{align}
%
It now follows with lemma~\ref{lem_cycle_index_theorem} that
%
\begin{align}
  \sum_{n=1}^\infty h_n t^n
  &=
  \sum_{\la} \frac{1}{z_\la}  t^{|\la|} \prod_{m=1}^{l(\la)} \theta_{\la_m}
  =
  \exp \left( \sum_{m=1}^\infty \frac{\theta_m}{m} t^m \right)
  =
  G_\Theta(t)
\end{align}
%
This proves \eqref{eq_def_gen_Gt_with_hn}.\\
%

%
If a generating function $g(t)$ is given then a natural question is:
what is $\nth{g}$ and what is the asymptotic behaviour of $\nth{g}$. If $g(t)$ is holomorphic near $0$ then one can use
Cauchy's integral formula to do this.
%
% Explicitly we have
% %
% \begin{align}
%   \nth{g} = \frac{1}{2\pi i} \oint_\gamma \frac{g(z)}{z^{n+1}}\ dz.
% \label{eq_cauchy_integral_formula}
% \end{align}
% %
% with $\gamma$ a simple closed curve with winding number $1$ about $0$.
% %
Unfortunately it is often difficult to calculate the integral explicit,
but there exists several theorems how to extract the asymptotic behaviour.
We now state such a theorem proven in \cite{hwang_thesis}. We first introduce some notation.

\begin{definition}
\label{def_delta_0}
Let $0< r < R$ and $0 < \phi <\frac{\pi}{2}$ be given. We then define
%
\begin{align}
\Delta_0 = \Delta_0(r,R,\phi) = \set{ z\in \C ; |z|<R, z \neq r ,|\arg(z-r)|>\phi}
\label{eq_def_delta_0}
\end{align}
%
\begin{figure}[ht!]
 \centering
 \includegraphics[width=.4\textwidth]{flajolet}
 \caption{Illustration of $\Delta_0$}
 \label{fig_delta_0}
\end{figure}
%
\end{definition}
%

\begin{definition}
 \label{def_function_class_F_alpha_r}
Let $g(t)$ and $\theta \geq 0, r>0$ be given. We then call $g(t)$ of class $\mathcal{F}(r,\theta)$ if
%
\begin{enumerate}
 \item there exists $R>r$ and $0 < \phi <\frac{\pi}{2}$ such that $g(t)$ is holomorphic in $\Delta_0(r,R,\phi)$,
 \item there exists a constant $K$ such that
   %
   \begin{align}
   g(t) = \theta \log\left( \frac{1}{1-t/r} \right) + K + O \left( t-r \right)   \text{ for } t\to r.
   \label{eq_class_F_r_alpha_near_r}
   \end{align}
   %
\end{enumerate}
%
We use to short notation $g(t) \in \mathcal{F}(r,\theta)$.
%
\end{definition}
%
We emphasize only the dependence on $\theta$ and $r$ since the other constants do not appear in the main results.
We now have
%
\begin{theorem}
\label{thm_hwang}
%
Let $F(t,w) = e^{w g(t)} S(t,w)$ be given. Suppose that
%
\begin{enumerate}
 \item Let $g(t)$ is of class $\mathcal{F}(r,\theta)$,
 \item \label{item_S_holo} $S(t,w)$ is holomorphic in $(t,w)$ for $|t| \leq r$ and  $|w| \leq \hat{r}$ for some $\hat{r}>0$, i.e. $S(t,w)$ is holomorphic in $(t,w)$ in a domain containing the set $\set{ (t,w)\in \C^2;  |t| \leq r, |w| \leq \hat{r} }$.
\end{enumerate}
%
Then
%
\begin{align}
  \nth{F(t,w)}
=
\frac{e^{Kw} n^{w\theta-1} }{r^n} \left(\frac{S(r,w)}{\Gamma(\theta w)} + O\left(  \frac{1 }{n}\right)\right)
\label{eq_thm_hwang}
\end{align}
%
uniform for $w \leq \hat{r} $ and with the same $K$ as in \eqref{eq_class_F_r_alpha_near_r}.
%
\end{theorem}
%

%
\begin{proof}
The idea of the proof is to take a suitable Hankel contour and to estimate the integral over each piece.
The details can be found in \cite[chapter 5]{hwang_thesis}.
\end{proof}
%
We use most times $w = 1$ and $S$ independent of $w$.
Singularity analysis is a very powerful tool. For example one can compute lower order error terms if one has more terms in the expansion of $g(t)$ near $r$. \\
%
A natural question at this position is: how can one prove that $g(t)$ is of class $\mathcal{F}(r,\theta)$?
It is most times easy to compute the radius of convergence of $g(t)$, but it is not obvious how to show that $g(t)$ is holomorphic in some $\Delta_0$. A possible tool to do this is

%
\begin{theorem}[Lindel\"ofs integral represention]
\label{thm_lindelof_integral_representation}
%
Let $\phi(z)$ be a holomorphic function for $\Re(z)>0$, satisfying
%
\begin{align}
 |\phi(z)| < C e^{A|z|} \text{ for } |z| \to \infty \text{ and }\Re(z)\geq \frac{1}{2} \text{ with some } A\in ]0,\pi[, C > 0 .
\end{align}
%
Let  $g(t):= \sum_{k=1}^\infty \phi(k) (-t)^k$. The radius of convergence of $g(t)$ is $e^{-A}$ and
%
%
\begin{align}
g(t)
=
\frac{-1}{2\pi i}
\int_{1/2 - i\infty}^{1/2 + i\infty}
\phi(z) t^z \frac{\pi}{\sin(\pi z)} \ dz.
\label{eq_lindelof_integral_representation}
\end{align}
%
Furthermore $g(t)$ can be holomorphically continued to the sector $-(\pi-A) < \arg(t) < (\pi-A)$.
%
\end{theorem}
%
\begin{proof}
See \cite[Theorem~2]{MR2578896}.
\end{proof}
%
Theorem~\ref{thm_lindelof_integral_representation} allows us in many situations to prove holomorphicity in a domain $\Delta_0$, but do not give any information about the behaviour of $g(t)$ near the singularity.
One way to compute the asymptotic behaviour of $g(t)$ near the singularity is to us the Mellin transform.
We do not introduce here the Mellin transform since this would lead us to far away from the topic of this paper.
We refer to \cite{MR1337752} for an introduction and to \cite[Section~3]{MR1678788} for an application to the polylogarithm.\\
%

Unfortunately we can not always apply Theorem~\ref{thm_lindelof_integral_representation} and the computation of the asymptotic behaviour near the singularity is often very difficult.
%Unfortunately it is not easy to prove or disprove if a function $g(t)$ is of class $\mathcal{F}(r,\theta)$.
An alternate approach is to combine singularity analysis with more elementary methods.
The idea is to write $F = F_1 F_2$ in a way that we can apply singularity analysis on $F_1$ and can estimate the growth rate of $\nth{F_2}$. One then can compute the coefficient $\nth{F}$ directly and apply elementary analysis on it. This method is called convolution method.
We now introduce a class where this approach is successful.
%
\begin{definition}
 \label{def_function_class_eF_alpha_r_gamma}
Let $g(t)$ and $\theta\geq 0, r>0, 0<\gamma \leq 1$ be given. We then call $g(t)$ of class $e\mathcal{F}(r,\theta,\gamma)$ if
%
\begin{align}
   g(t) = \theta \log\left( \frac{1}{1-t/r} \right) + g_0(t)   \text{ for } t\to r \text{ with }\nth{g_0} = O(r^{-n} n^{-1-\gamma}).
   \label{eq_class_eF_alpha_r_gamma_near_r}
\end{align}
%
\end{definition}
%
%
\begin{theorem}
\label{thm_hwang_2}
%
Let $F(t,w) = e^{w g(t)} S(t,w)$ be given such that
%
\begin{enumerate}
 \item  $g(t)$ is of class $e\mathcal{F}(r,\theta,\gamma)$,
 \item   $S(t,w)$ is holomorphic in $(t,w)$ for $|t| \leq r$ and  $|w| \leq \hat{r}$ for some $\hat{r}>0$.
\end{enumerate}
%
We then have
%
\begin{align}
\nth{F(t,w)}
=
\frac{e^{w K} n^{w\theta-1} }{r^n} \frac{S(r,w)}{\Gamma(\theta w)} + R_n(w)
\end{align}
%
with $K = (g_0(r))$ and
%
\begin{align}
  R_n(w)
  =
  \left\{
    \begin{array}{ll}
      O \left(\frac{n^{\theta\Re(w) - 1- \gamma} \log(n)}{r^n} \right), & \hbox{ if }\Re(w) \geq 0 \\
      O \left(\frac{ n^{-1 - \gamma} }{r^n} \right), &  \hbox{ if } \Re(w) < 0.
    \end{array}
  \right.
\end{align}
%
uniformly for bounded $w$.
%
\end{theorem}
%
\begin{proof}
See \cite{MR1724562}.
\end{proof}
%







%
We now can compute the asymptotic behaviour of $h_n$.
%
\begin{lemma}
\label{lem_asymptotic_hn}
Let $g_\Theta(t)$ be of class $\mathcal{F}(r,\theta)$ or of class $e\mathcal{F}(r,\theta,\gamma)$. We then have
%
\begin{align}
\frac{1}{h_n}
\sim
r^n \frac{\Gamma(\theta)}{e^{K} n^{\theta-1}}.
\label{eq_asymptotic_hn}
\end{align}
%
with the same $K$ as in \eqref{eq_class_F_r_alpha_near_r} resp. as in Theorem~\ref{thm_hwang_2}.
%
\end{lemma}

\begin{proof}
We have proven that $\sum_{n=0}^\infty h_n t^n = G_\Theta(t) = \exp( g_\Theta(t))$.
We thus can apply Theorem~\ref{thm_hwang} resp. Theorem~\ref{thm_hwang_2} with $g(t) = g_\Theta(t)$ for $w=1$ and $S(t,w) \equiv 1$. We get
%
\begin{align}
  h_n
% \ \sim \
% \sum_{j=1}^k \xi_j^{-n} \frac{n^{\theta_j-1}}{\Gamma(\theta_j)}
% \ \sim \
% r^{-n} e^{c_1} \frac{n^{\theta_1-1}}{\Gamma(\theta_1)}
\sim
\frac{e^K n^{\theta-1}}{r^n \Gamma(\theta)}
\end{align}
%
\end{proof}
%

\textbf{Remark:}

There exists several other versions of the Theorems~\ref{thm_hwang} and Theorems~\ref{thm_hwang_2}.
For example one can replace $\log(1-t/r)$ by other functions (see \cite{Flajolet_generating}) or allow more than one singularity (see \cite[chapter VI.5]{FlSe09}.



